Adaptive Federated Learning with Functional Encryption: A Comparison of Classical and Quantum-safe Options

Federated Learning (FL) is a collaborative method for training machine learning models while preserving the confidentiality of the participants' training data. Nevertheless, FL is vulnerable to reconstruction attacks that exploit shared parameters to reveal private training data. In this paper, we address this issue in the cybersecurity domain by applying Multi-Input Functional Encryption (MIFE) to a recent FL implementation for training ML-based network intrusion detection systems. We assess both classical and post-quantum solutions in terms of memory cost and computational overhead in the FL process, highlighting their impact on convergence time.

==> sections/Aknowledgment.tex <==
\section*{Acknowledgment}
This work was supported by Ministero delle Imprese e del Made in Italy (IPCEI Cloud DM 27 giugno 2022 – IPCEI-CL-0000007) and European Union (Next Generation EU).

==> sections/Preliminaries.tex <==
\section{Preliminaries}
We start by presenting two notions of security we based our schemes on. A detailed description is out of the scope of this paper and we invite the reader to check \cite{fromseltoadpt} and \cite{fully_secure} for an exhaustive and formal presentation of the topic.

\emph{Adaptive Security}. We say that a scheme is \textit{adaptively secure} if it is resistant against 
adaptive attacks, i.e. where the attacker is allowed to choose the pair of messages in the challenge phase, based on the previously collected
information.

\emph{Selective Security}. We say that a scheme is \textit{selectively secure} if it is resistant against selective
attacks, i.e. where the attacker has to declare the pair of challenge messages at
the outset of the game (that is, before seeing the master public key). In this setting, there is no previous information the attacker can use. 

Of course, the adaptive security notion is stronger than the selective one, having an attacker modeled by more realistic features. Still, adaptively secure schemes are generally less efficient than selectively secure ones, and the latter may as well be feasible for some settings. The choice between these two levels of security comes off as a classic evaluation of the tradeoff between security and performance we are inclined to sustain.


Furthermore, we hereby give a useful presentation of the two main algorithms of FLAD. Notation should be clear from the context and further explanation of symbols and procedures are given in the following.

\begin{algorithm}
\caption{Adaptive federated learning process}
\label{alg: FLAD}
\begin{algorithmic}[1]
\Require Global model ($w_0$), set of clients ($C$)
\Procedure{AdaptiveFederatedTraining}{}
    \State $a_{\text{max}} \gets 0$ \Comment{Max accuracy score}
    \State $sc \gets 0$ \Comment{Early stop counter}
    \State $C_0 \gets C$
    \State $c_e = e_{\text{max}}, c_s = s_{\text{max}} \quad \forall c \in C_0$ \Comment{Epochs and steps}
    \State $c \gets \text{InitClients}(w_0, c_e, c_s) \quad \forall c \in C_0$
    \For{$t = 1, 2, 3, \dots$}
        \Comment{Federated training loop}
        \ForAll{$c \in C_{t-1}$} \Comment{In parallel}
            \State $w_t^c \gets \text{ClientUpdate}(w_{t-1}, c_e, c_s)$
        \EndFor
        \State $w_t = \frac{1}{|C|} \sum_{c=1}^{|C|} w_t^c$ \Comment{Arithmetic mean}
        \State $a^\mu \gets [a^c]_{c \in C} \gets \text{SendModel}(w_t, C)$
        \If{$a^\mu > a_{\text{max}}$}
            \State $\bar{w} \gets w_t$ \Comment{Save best model}
            \State $a_{\text{max}} \gets a^\mu$ \Comment{Save max accuracy score}
            \State $sc \gets 0$ \Comment{Reset early stop counter}
        \Else
            \State $sc \gets sc + 1$
        \EndIf
        \If{$sc > \text{patience}$}
            \State \text{SendModel}($\bar{w}, C$) \Comment{Send final model}
            \State \Return \Comment{End of the process}
        \Else
            \State $C_t \gets \text{SelectClients}(C, [a^c]_{c \in C}, a^\mu)$
        \EndIf
    \EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}
In \Cref{alg: FLAD}, "patience" is an arbitrary threshold of rounds with no accuracy improvement, \textsc{SendModel} is an implicit algorithm that expresses the process of sending the model from the client to the aggregator, \textsc{ClientUpdate} is the local training algorithm of the specific client and \textsc{SelectClients} (\Cref{alg: SelectClients}) is the algorithm run by the aggregator in order to choose the set of clients which will train in the next round.
\begin{algorithm}
\caption{Select the clients for the next round of training}
\label{alg: SelectClients}
\begin{algorithmic}[1]
\Require Clients ($C$), accuracy scores ($[a^c]_{c\in C}$), average accuracy score ($a^\mu$)
\Ensure List of selected clients ($C'$)
\Procedure{SelectClients}{$C$, $[a^c]_{c\in C}$, $a^\mu$}
    \State $C' \gets \{c \in C \mid a^c \leq a^\mu\}$
    \State $a \gets \min_{c \in C'}(a^c)$
    \State $\bar{a} \gets \max_{c \in C'}(a^c)$
    \ForAll{$c \in C'$}
        \State $\sigma = \frac{\bar{a} - a^c}{\bar{a} - a}$ \Comment{Scaling factor}
        \State $c_e = e_{\min} + (e_{\max} - e_{\min}) \cdot \sigma$
        \State $c_s = s_{\min} + (s_{\max} - s_{\min}) \cdot \sigma$
    \EndFor
    \State \Return $C'$
\EndProcedure
\end{algorithmic}
\end{algorithm}
